Navigating with Graph Representations for Fast and Scalable Decoding of Neural Language Models

Neural language models (NLMs) have recently gained a renewed interest by achieving state-of-the-art performance across many natural language processing (NLP) tasks. However, NLMs are very computationally demanding largely due to the computational cost of the softmax layer over a large vocabulary. We observe that, in decoding of many NLP tasks, only the probabilities of the top-K hypotheses need to be calculated preciously and K is often much smaller than the vocabulary size. This paper proposes a novel softmax layer approximation algorithm, called Fast Graph Decoder (FGD), which quickly identifies, for a given context, a set of K words that are most likely to occur according to a NLM. We demonstrate that FGD reduces the decoding time by an order of magnitude while attaining close to the full softmax baseline accuracy on neural machine translation and language modeling tasks. We also prove the theoretical guarantee on the softmax approximation quality.

==> backup/spacing.tex <==
\iftoggle{tech-report}{%
}{
\renewcommand{\baselinestretch}{0.96}
}

\setlist{nosep} % Change space between items in a listing.
\setlength{\textfloatsep}{5pt} % Control space after figure and before text. 
\setlength{\dbltextfloatsep}{5pt}

\usepackage{titlesec}
\usepackage{setspace}

\newlength{\sectionbelowskip}
\newlength{\sectionaboveskip}
\newlength{\subsectionbelowskip}
\newlength{\subsectionaboveskip}
\newlength{\subsubsectionbelowskip}
\newlength{\subsubsectionaboveskip}
\newlength{\paragraphaboveskip}

%  Control space before and after table
\newcommand{\spaceabovetable}{\vspace*{-1em}}
\newcommand{\spacebelowtable}{\vspace*{-1em}}


\newcommand{\setvspace}[2]{%
  #1 = #2
  \advance #1 by -1\parskip}

% Ever so slightly tighter than defaults:
\setlength{\sectionbelowskip}{3pt}
\setvspace{\sectionaboveskip}{3pt}
\setlength{\subsectionbelowskip}{3pt}
\setvspace{\subsectionaboveskip}{3pt}
\setlength{\subsubsectionbelowskip}{1pt}
\setvspace{\subsubsectionaboveskip}{2pt}
\setvspace{\paragraphaboveskip}{2pt}

\titlespacing*{\section}{0pt}{\sectionaboveskip}{\sectionbelowskip}
\titlespacing*{\subsection}{0pt}{\subsectionaboveskip}{\subsectionbelowskip}
\titlespacing*{\subsubsection}{0pt}{\subsectionaboveskip}{\subsectionbelowskip}
\titlespacing*{\paragraph}{0pt}{\paragraphaboveskip}{*}

\titleformat{\subsubsection}
  {\normalfont\normalsize\bfseries}{\thesubsubsection}{1em}{}
\titlespacing*{\subsubsection}{0pt}{\subsubsectionaboveskip}{\subsubsectionbelowskip}

\makeatletter % Control space around theorem and lemma
\def\thm@space@setup{%
  \thm@preskip=3pt
  \thm@postskip=\thm@preskip % or whatever, if you don't want them to be equal
}
\makeatother

\makeatletter % Control the space around the proof.
\renewenvironment{proof}[1][\proofname]{\par
  \vspace{1pt}% remove the space after the theorem
  \pushQED{\qed}%
  \normalfont
  \topsep0pt \partopsep0pt % no space before
  \trivlist
  \item[\hskip\labelsep
        \itshape
    #1\@addpunct{.}]\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
  \addvspace{3pt plus 3pt} % some space after
}
\makeatother 

==> discussion.tex <==
\section{Discussion and Future Work}
\label{sec: discussion}

\paragraph{Compatibility.} Our proposed approach is complementary to many existing work. A model can be trained with sampling-based approach~\cite{strategies-training-large-vocabulary-nn, on-very-large-target-vocab-for-nmt, noise-contrastive-estimation, negative-sampling, self-normalisation}, and \SWVG can improve the inference time of those trained models. \SWVG is applicable to SVD-softmax~\cite{svd-softmax}, where top K most probable words in the preview window can be found through \SWVG.
\minjia{TODO: Talk about compatibility with other approaches, such as hierarchical softmax etc.}

\paragraph{SWVG as an evolving dynamic graph.} The SWVG in the paper investigated is static, which means it works on any pre-trained models. However, human language is certainly an evolving system, where its present structure is determined by its past evolution. One future direction is that we treat SWVG as a growing network of interacting words. New interactions between words emerge from time to time in the learning phase, and new edges can be constructed. Once the training has finished, the learned SWVG can be readily used for serving.

\paragraph{Generalization and connection with prior work.}

Based on Definition~\ref{defn: retrieval-topk}, we can pose the vocabulary projection problem as finding $K$ highest ranked words in Euclidean spaces. This means it is possible to substitute $CreateSwvg$ (line~\ref{lst:transformation:createHnswIndex} in Algorithm~\ref{algo: transformation}) with other structures to encode relationships between words.
% and replace $SearchSwvg$ (line~\ref{lst:inference:search} in Algorithm~\ref{algo: inference}). 
Many classical K-ANN algorithms may apply~\cite{kd-tree, vp-tree,locality-sensitive-hashing,locality-preserving-hashing}. This is a direction that can be investigated as future work. 
% Here we review the applicability of a few of them.
% We review a few which have been applied extensively. The key idea of K-ANN algorithms is to find the NN with high probability "only", instead of probability 1. 
% Most of the effort on k-ANN has been devoted to the Euclidean distance, though recent generalizations have been proposed for other metrics~\cite{} and non-metrics~\cite{}. 
% We review a few which have been applied extensively. 

% One large category of K-ANN algorithms are based on the idea of space partitioning, such as KD-tree~\cite{kd-tree} and VP-tree~\cite{vp-tree}. These approaches work well in low dimensions, \eg, less than 15, (search complexity is close to $O(\log{N}))$, but context vector in deep learning models often have much higher dimensions and their effectiveness quickly decreases as the dimensionality grows. The complexity of these approaches is $O(d \cdot N^{1-1/d})$~\cite{worst-case-kdtree}, which is not more efficient than the brute-force exhaustive distance computation at high dimension. Another family of popular K-ANN algorithms is Locality Sensitive Hashing (LSH) based approaches~\cite{locality-sensitive-hashing}. These methods map a high-dimensional point to a low-dimensional hash value (\eg, bucket) via a set of locality preserving hash functions~\cite{locality-preserving-hashing, lsh-2004}. Methods in this category enjoy sound probabilistic theoretical guarantees on the query results quality and search efficiency in the worst case. However, in practice, the performance of LSH degrades on datasets with large variations in density, due to the uneven distribution of points across buckets. As a result, LSH based approach often requires data-dependent hashing schemes to exploit data distribution in order to get high accuracy~\cite{optimal-data-dependent-hashing}. This is a direction that can be investigated as future work. 

More generally, our \SWVG approach can be applied to other models with large \projection, such as image classification tasks with large output projection layers~\cite{}. Our \NIET transformation allows us to leverage any nearest neighbor search algorithm defined in metric space to efficiently solve the inference bottleneck of \projection problem.

% \paragraph{Memory usage} 
% \swgp does not require both the original embedding vectors and the graph structure. Embeddings are nested in graph nodes.
% \minjia{Mentioned when introducing \SWVG.}

\paragraph{Metric learning.} Instead of using \NIET and measuring the closeness between words using the general--purpose Euclidean distance, it is also possible to automatically learn a metric that rank word pairs higher if they are indeed semantically close with \emph{metric learning}~\cite{metric-learning-survey}. Further improvement on the results is expected when the metric is designed specifically for each task at hand.

\paragraph{Expanding vocabulary coverage.} It has been observed that tasks such as NMT rapidly degrade their performance as the number of unknown words increases~\cite{properties-of-nmt, rnn-machine-translation}. Our approach models vocabulary projection as \SWVG without incurring a linear increase of the inference time, which potentially allows tasks to handle larger vocabulary and mitigate the OOV (Out-Of-Vocabulary) ratio. 
% It is also complementary to vocabulary selection method

% \paragraph{End-to-end}

% Our current approach does not require retraining of the model. Learn the Euclidean representation end-to-end, such that Euclidean distance between word embeddings reflects semantic similarity. Future work.


% \paragraph{Vocabulary selection.} and other techniques that target at reducing the vocabulary size.
% \minjia{Does vocabulary selection work only under NMT? Our approach seems to be complementary.}



==> extra.tex <==
\section{Visualization of Similarity Relation}
Our \NIET approach provides a convenient way to transform inner product against word embedding vectors to a metric space, exploiting closeness between words through their metric relation, and then inversely transforming metric distance back to inner product result in $O(1)$ complexity, which then can be consumed by the final softmax function to compute word probabilities. To see the metric relation, we utilize t-SNE~\cite{t-sne}
% \footnote{http://scikit-learn.org}
to visualize the weights at the vocabulary projection layer by mapping it to a 2D Euclidean distance space. As shown in Figure~\ref{fig:freq_word2vec}, words in the projection layer clearly has conceptual and positional properties.
Thus semantic more similar words are closer in distance. 

\begin{figure}[H]
\centering 
\includegraphics[width=0.7\linewidth]{figs/freq_word2vec}
\caption{Projection of word embedding vectors on a 2D Euclidean distance space. 400 words are sampled from the vocabulary projection weights of WikiText-2 by filtering the high frequency words (higher than 1000) and low frequency words (less than 100). Training methodology to get the weights is included in Section~\ref{subsec: eval-lm}.}
\label{fig:freq_word2vec}
\end{figure} 

\section{Finding Top-$K$ Minimum Subset Through Inner-Product is Equivalent to Optimizing 1-Lipschitz Functions on Small World Graphs}
\label{subsec: equivalence}

% \minjia{TODO: Decide whether MIPS is a better term for describing vocabulary projection. \minjia{Decoding is a bit better.}}

% In this section, we establish the equivalence of the top-$K$ projection softmax probability problem and the top-$K$ minimum search problem for a matching function on SWVG. Briefly, we identify the set of vocabulary as the set of nodes. For each pair of nodes we define a distance metric which is compatible with the projection embeddings of the vocabulary. That is, if two words in the vocabulary are semantically similar, one expects their distance to be smaller.Based on the distance metric defined on the nodes, we impose a set of edges which turns it into a small world graph. We also define a matching function for each pair of word and context vector. We show that the matching function satisfies Lipschitz condition, and it is monotonic in terms of the projection softmax probability. The Lipschitz condition allows the hierarchical small word graph construction to solve the top-$K$ minimum search problem effectively. Moreover, the monotonicity implies the equivalence of the top-$K$ projection softmax problem and the top-$K$ minimum search problem on SWVG.

% Let $V$ be the set of vocabulary. 
By a metric on $V$ it indicates a function $\rho: V\times V\longrightarrow\mathds{R}_{\geq 0}$ such that the following conditions hold: (1) $\forall v_1, v_2\in V$, $\rho(v_1, v_2) \geq 0$, and $\rho(v_1, v_2) = 0$ iff $v_1 = v_2$; (2) $\forall v_1, v_2\in V$ $\rho(v_1, v_2) = \rho(v_2, v_1)$; and (3) $\forall v_1, v_2, v_3\in V$, $\rho(v_1, v_2) + \rho(v_2, v_3) \geq \rho(v_1, v_3)$. Namely, $\rho$ is a distance metric defined on $V$.

We say that $\mu: V\times\mathds{R}^d\longrightarrow\mathds{R}$ is a matching function, if $\mu_h := \mu(\cdot, h)$ is 1-Lipschitz on the metric space $(V, \rho)$ for any context vector $h\in\mathds{R}^d$. That is, $\forall x_1, x_2\in V$, $|\mu_h(x_1) - \mu_h(x_2)|\leq \rho(x_1, x_2)$. 

For a matching function $\mu$ and $h\in\mathds{R}^d$, we say that $V'\subseteq V$ is a top-$K$ minimum subset for $h$ under $\mu$, if $|V'| = K$ and $\mu(x, h) \leq \mu(x', h)$ for all $x\in V'$ and $x'\in V-V'$. 

\begin{theorem}
Let $V$ be the set of word vocabulary, and $E = [W; b]$ be the augmented projection embedding matrix, where $W$ is the projection weights, and $b$ is the projection bias. Denote by $w_i$ ($b_i$) the corresponding weight vector (bias) for $i$-th word. Then there exists a metric $\rho$ on $V$ and a non-zero matching function $\mu$ such that for any context vector $h\in\mathds{R}^d$, the top-$K$ words found by projection with respect to $h$ is the same as the $K$-minimum subset for $h$ under $\mu$. Moreover, let $U$ be the 2-norm of $E$. One such metric is $\rho(x_i, x_j) = \sqrt{\|w_i - w_j\|_2^2 + |b_i - b_j|^2 + \left(\sqrt{U^2 - \|w_i\|^2 - b_i^2} - \sqrt{U^2 - \|w_j\|_2^2 - b_j^2}\right)^2}$, and the corresponding $\mu$ can be chosen as $\mu(x_i, h) = \sqrt{U^2 + \|h\|_2^2 - 2(w_i^Th + b_i)}$.
\end{theorem}
\begin{proof}
We prove this theorem in three steps. First we verify that that the $\rho$ defined in the theorem is indeed a distance metric on $V$. Next we show that $\mu$ is 1-Lipschitz on $V$ with respect to $\rho$. Finally we will show the equivalence of the finding top-$K$ minimum subset through inner-product and minimization of $\mu$ on $V$.

We start with verifying that $\rho$ is a distance metric. To see this, we identify each word $x_i\in V$ with a vector $z_i\in\mathds{R}^{d+2}$, which is $z_i := [w_i;b_i;\sqrt{U^2 - \|w_i\|_2^2 - b_i^2}]$. Since $U$ is the 2-norm of the augmented weight matrix, the vector $z_i$ is well defined for all $x_i\in V$. Note that $\rho(x_i, x_j)$ defined in the theorem is simply the Euclidean distance between the vectors $z_i$ and $z_j$ in $\mathds{R}^{d+2}$. This shows that $\rho$ is indeed a distance metric.

\minjia{Are we using Euclidean distance to prove $\rho$ is a metric? That sounds to me like a circular reasoning. Also, how do we know that $\rho$ is a metric? Shouldn't we prove it by demonstrating how it satisfies the four properties of being a metric? }

To see that $\mu$ is 1-Lipschitz, we note that for any context vector $h\in\mathds{R}^d$, we identify a vector $\tilde h = [h;1;0]\in\mathds{R}^{d+2}$. Now one verifies by simple computation that $\mu(x_i, h)$ is the Euclidean distance between $z_i$ and $\tilde h$ in $\mathds{R}^{d+2}$. The triangular inequality then implies that $\mu$ is 1-Lipschitz on $V$ with respect to $\rho$.

To see that the finding top-$K$ minimum subset through inner-product is equivalent to finding the top-$K$ minimum subset of $\mu$ on $V$, simply note that $\mu(x_i, h)$ is monotonically decreasing in $w_i^Th + b_i$.
\end{proof}

% Talk about smoothing.
% \subsection{Probability Redistribution via Smoothing}
\section{Rank-consistent Smoothing}
\label{subsec: smoothing}


\minjia{With the new storyline, especially with a focus on solving the top K softmax problem, this part can be put into the appendix or perhaps even removed. \xiaodl{If we remove this section, we also need to remove its corresponding claims in the previous content}}

In \SWVG, nodes unvisited do not have their Euclidean distance readily available. How should the probability of those words be assigned? We could take a "winners take all" approach and distribute probability among top $K$ highest ranked words and assign a very small probability $\epsilon$ to the rest, which may already suffice for most applications, but there is nothing interesting to say about their relative quality.  
% Recent studies have proven that Laplace smoothing is more effective than other probability smoothing methods in language-model-based pseudo-relevance feedback and recommender systems~\cite{laplace-smoothing-pseudo-relevance, laplace-smoothing-recommender-system}. 
We note that this problem is similar, in some respects, to the \textbf{unseen n-grams} problem in count-based language modeling, where many \emph{smoothing regularization} techniques have been introduced~\cite{study-of-smoothing}. 
% Smoothing technique has recently seen its use in modern neural networks as well~\cite{rethink-inception-architecture}. 
A straightforward way 
% One of such techniques
% way to do smoothing 
is to apply Laplacian smoothing, which builds prior knowledge of word frequency in the training dataset~\cite{laplacian-smoothing} and smooth a probability distribution $y$ via:
\begin{eqnarray}
   &\tilde y_i = \frac{y_i + \epsilon \cdot f_i}{1 + \epsilon}&
\end{eqnarray}
where $y$ can be sparse
% logits of size $|V|$ in which 
(\ie, some positions have 0s), $f_i$ the frequency of word $w_i$ in the training dataset, and $\epsilon$ a hyperparameter, which can be
% is a small value that can be 
tuned on the development dataset.
% Recent studies have proven that Laplacian smoothing is more effective than other probability smoothing methods in language-model-based pseudo-relevance feedback and recommender systems~\cite{laplace-smoothing-pseudo-relevance, laplace-smoothing-recommender-system}. 
% One way to smooth the vocabulary distribution is by computing:


In our work we propose a modified approach: in those applications where top-$K$ vocabulary matters most, we want to retain the order so that the top-$K$ vocabulary after smoothing remains unchanged. More precisely, we want the following. 

\begin{defn}
Let $\mathcal K$ denote the top $K$ indices of vocabulary. Let $\{y_i\}$ be a probability distribution supported on $K$. A smoothing $\tilde y_i$ from $y_i$ is called \emph{consistent}, if the following conditions are satisfied: (1) for any $i$, $\tilde y_i > 0$; (2) for any $i, j\in\mathcal K$, $y_i \leq y_j$ iff $\tilde y_i \leq \tilde y_j$; and (3) $\tilde y_i \geq \tilde y_j$ for any $i\in\mathcal K$ and $j\not\in\mathcal K$. 
\end{defn}

Note that the vanilla Laplacian smoothing may not be consistent. We use the following modified smoothing mechanism that is consistent. 

\begin{theorem}
Suppose $y_i > 0$ for $i\in\mathcal K$. Let $f_i$ be the prior probability distribution (frequency) of the vocabulary such that $f_i > 0$ for all $i$. Then there exists a consistent smoothing of $y_i$. Denote by $g_i$ the conditioning of $f_i$ on $V\backslash \mathcal K$, i.e., $g_i = \frac{f_i}{\sum_{i\not\in \mathcal K} f_i}$ if $i\not\in \mathcal K$ and $g_i = 0$ otherwise. One such consistent smoothing is given by 
\begin{equation}
\tilde y_i = \frac{y_i + \epsilon g_i}{1 + \epsilon},
\end{equation}
where $0 < \epsilon < \min_{i\in\mathcal K} y_i$.
\end{theorem}
\begin{proof}
It suffices to verify the three conditions for consistent smoothing. First note that $y_i > 0$ for $i\in\mathcal K$ and $g_i > 0$ for $i\not\in\mathcal K$, thus $\tilde y_i > 0$ for all $i$. Now assume $i, j\in\mathcal K$, with $y_i \leq y_j$. Since $i$ and $j$ are among top $K$, we have $g_i = g_j = 0$. Thus $\tilde y_i = \frac{y_i}{1 + \epsilon} \leq \frac{y_j}{1 + \epsilon} = \tilde y_j$. Finally, choose $i\in\mathcal K$ and $j\not\in\mathcal K$. It follows that $\tilde y_i = \frac{y_i + \epsilon g_i}{1 + \epsilon} \geq \frac{\min_{i\in\mathcal K} y_i}{1 + \epsilon} \geq \frac{\epsilon}{1 + \epsilon} \geq \frac{\epsilon g_j}{1 + \epsilon} = \tilde y_j$. 
\end{proof}

==> impl.tex <==
\section{Implementation}
\label{sec:implementation}




==> related.tex <==
\section{Related Work}
\label{sec: related-work}

In this section, we explain how the complexity of the vocabulary projection is addressed by existing approaches for both the training and inference phase.
% Prior work often combine the vocabulary projection together with the softmax function and optimize it as a whole (as in Equation~\ref{eqn: vocabulary_projection}). 
They fall into several camps in terms of how they speedup this computation~\footnote{Online article~\cite{softmax-approximation} also provides a good summary of different approaches.}:
\paragraph{(1) Sampling--based approaches:} These approaches speedup the computation of vocabulary projection including the softmax function by approximating the normalization in the denominator of the softmax through sampling and training only on a small subset of possible outputs. Approaches in this category include importance sampling~\cite{strategies-training-large-vocabulary-nn}, target sampling~\cite{on-very-large-target-vocab-for-nmt}, noise contrastive estimation~\cite{noise-contrastive-estimation}, negative sampling~\cite{negative-sampling}, self--normalisation~\cite{self-normalisation} etc. The issue with sampling--based approaches is that they speedup only training but not inference. 
% Noise contrastive estimation (NCE), Gutmann et al. (AISTATS 2010)
% Negative sampling,  Mikolov et al. (arXiv 2013)
% Limitation: speed-up only training not inference.

\paragraph{(2) Hierarchical--softmax/CNN--softmax/LSTM--softmax:} These approaches modify the structure of the the projection layer to improve its efficiency. Hierarhical--softmax speeds up training significantly but not inference~\cite{hierarchical-softmax}. CNN--softmax and LSTM--softmax compress the parameters in the projection layer but does not offer any training nor inference speedup~\cite{explore-the-limits-of-lm}.  
% the Devlin et al. (ACL 2014)
% Limitation: does not reduce the cost of projection, only avoid the cost of softmax computation. Our technique is complimentary to self-normalisation  
% \paragraph{NN approximation}
% CNN-softmax / LSTM-softmax, Rafal et al. 2016
% Limitation: reduce memory footprint, but does not reduce projection speed

% \paragraph{Hierarchical softmax and its variant} (Morin, F., \& Bengio, AISTATS 2005)
% Limitation: Speed-up only training

\paragraph{(3) Differentiated softmax/SVD-softmax:} Both approaches can speedup the inference. Differentiated softmax improves inference speed by storing the projection weights as a sparse weight matrix~\cite{strategies-training-large-vocabulary-nn}. However, the word representations are restricted from the start (based on frequency), limiting its expressiveness. SVD--softmax is the state-of-the-art approach on improving the inference speed of vocabulary projection. 
It approximates the projection weights through SVD (singular vector decomposition) and a refinement of probable top-$\bar{V}$ words~\cite{svd-softmax}. It brings the complexity from $O(|V| \times D)$ to $O(|V| \times \bar{D} + |\bar{V}| \times D)$, where $\bar{D}$ indicates the preview window size. The issue with this approach is that its complexity is still proportional to the size of the vocabulary, limiting its scalability.
\xiaodl{We can use $\bar{V}$ and $\bar{D}$ to indicate top-W words and preview window size, which is a sub set of $V$ and $D$, respectively.}
 %It approximates the projection weights through SVD (singular vector decomposition) and a refinement of probable top-$W$ words~\cite{svd-softmax}. It brings the complexity from $O(|V| \times D)$ to $O(|V| \times W + N \times D)$. The issue with this approach is that its complexity is still proportional to the size of the vocabulary, limiting its scalability.

% \paragraph{SVD-softmax} (state-of-the-art), Shim NIPS 2017
% Reduce O(V x D) to O (V x W + N x D)
% The drawback for the SVD-softmax is that it has a part of search algorithm with a linear vocabulary size scaling.
% Difference with our approach: O (V x D) to O (log(V) x D)

% \paragraph{Vocabulary selection}
% Reduce word vocabulary size (still doing full softmax). 
% Used specifically in machine translation? Complementary to our work?
% Does not address OOV issue. Limited expressiveness. Complimentary to our work



